Anderson Mixing in Bures Wasserstein Space of Gaussian Measures

Various statistical tasks, including sampling or computing Wasserstein barycenters, can be reformulated as fixed-point problems for operators on probability distributions. Accelerating standard fixed-point iteration schemes provides a promising novel approach to the design of efficient numerical methods for these problems. The Wasserstein geometry on the space of probability measures, although not precisely Riemannian, allows us to define various useful Riemannian notions, such as tangent spaces, exponential maps and parallel transport, motivating the adaptation of Riemannian numerical methods. We demonstrate this by developing and implementing the Riemannian Anderson Mixing (RAM) method for Gaussian distributions. The method reuses the history of the residuals and improves the iteration complexity, and we argue that the additional costs, compared to Picard method, are negligible. We show that certain open balls in the Bures-Wasserstein manifold satisfy the requirements for convergence of RAM. The numerical experiments show a significant acceleration compared to a Picard iteration, and performance on par with Riemannian Gradient Descent and Conjugate Gradient methods.

==> tab/BC_max_min_acc.tex <==
\begin{tabular}{lrrrr}
\toprule
$n_{\sigma}$ & $3.0$ & $5.0$ & $10.0$ & $20.0$ \\
$d$ &  &  &  &  \\
\midrule
2 & $0.98$ & $1.29$ & $1.36$ & $1.25$ \\
3 & $1.00$ & $1.44$ & $1.34$ & $1.37$ \\
5 & $1.27$ & $1.33$ & $1.39$ & $1.36$ \\
10 & $1.61$ & $1.52$ & $1.57$ & $1.40$ \\
20 & $1.87$ & $1.76$ & $1.70$ & $1.52$ \\
50 & $1.77$ & $1.95$ & $1.56$ & $1.51$ \\
\bottomrule
\end{tabular}


==> tab/BC_n_steps_by_method.tex <==
\begin{tabular}{llrrrr}
\toprule
 &  & Picard & RGD & BWRAM & RCG \\
$d$ & $n_{\sigma}$ &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{3} & 3 & 6.2 & 14.4 & \bfseries 5.4 & 31.6 \\
 & 5 & 9.8 & 16.6 & \bfseries 7.0 & 29.0 \\
 & 10 & 8.6 & 15.8 & \bfseries 6.8 & 28.6 \\
 & 20 & 9.0 & 15.2 & \bfseries 6.6 & 26.2 \\
\cline{1-6}
\multirow[c]{4}{*}{5} & 3 & 9.8 & 18.0 & \bfseries 7.4 & 32.4 \\
 & 5 & 9.6 & 18.2 & \bfseries 7.2 & 34.8 \\
 & 10 & 10.6 & 18.8 & \bfseries 7.4 & 38.4 \\
 & 20 & 10.0 & 19.0 & \bfseries 7.2 & 36.0 \\
\cline{1-6}
\multirow[c]{4}{*}{10} & 3 & 13.6 & 19.2 & \bfseries 8.6 & 26.4 \\
 & 5 & 13.8 & 20.4 & \bfseries 9.0 & 33.4 \\
 & 10 & 13.8 & 22.6 & \bfseries 8.8 & 40.6 \\
 & 20 & 11.2 & 22.0 & \bfseries 8.0 & 39.4 \\
\cline{1-6}
\multirow[c]{4}{*}{20} & 3 & 20.6 & 23.8 & \bfseries 10.6 & 34.6 \\
 & 5 & 19.0 & 21.6 & \bfseries 11.2 & 36.6 \\
 & 10 & 17.0 & 22.8 & \bfseries 10.0 & 44.6 \\
 & 20 & 13.4 & 21.8 & \bfseries 8.8 & 44.8 \\
\cline{1-6}
\multirow[c]{4}{*}{50} & 3 & 26.4 & 30.8 & \bfseries 13.4 & 37.2 \\
 & 5 & 23.8 & 29.2 & \bfseries 12.8 & 50.2 \\
 & 10 & 18.6 & 27.4 & \bfseries 11.2 & 44.4 \\
 & 20 & 14.2 & 26.4 & \bfseries 9.2 & 44.0 \\
\cline{1-6}
\bottomrule
\end{tabular}


==> tab/EntBC_n_steps_by_method.tex <==
\begin{tabular}{llrrrr}
\toprule
 &  & Picard & RGD & BWRAM & RCG \\
$d$ & $n_{\sigma}$ &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{3} & 3 & 6.6 & 8.8 & \bfseries 4.4 & 15.8 \\
 & 5 & 10.6 & 9.0 & \bfseries 5.8 & 12.2 \\
 & 10 & 10.4 & 9.8 & \bfseries 4.8 & 16.4 \\
 & 20 & 9.2 & 10.0 & \bfseries 5.0 & 13.4 \\
\cline{1-6}
\multirow[c]{4}{*}{5} & 3 & 8.8 & 9.0 & \bfseries 6.4 & 14.2 \\
 & 5 & 8.2 & 9.8 & \bfseries 5.6 & 15.8 \\
 & 10 & 9.0 & 10.6 & \bfseries 6.0 & 17.0 \\
 & 20 & 9.4 & 10.8 & \bfseries 5.0 & 18.4 \\
\cline{1-6}
\multirow[c]{4}{*}{10} & 3 & 14.2 & 8.6 & \bfseries 7.0 & 9.0 \\
 & 5 & 13.2 & 11.2 & \bfseries 6.2 & 14.0 \\
 & 10 & 11.0 & 12.6 & \bfseries 6.6 & 15.6 \\
 & 20 & 11.4 & 11.0 & \bfseries 5.4 & 16.2 \\
\cline{1-6}
\multirow[c]{4}{*}{20} & 3 & 23.2 & 11.4 & \bfseries 7.8 & 11.2 \\
 & 5 & 23.8 & 11.0 & \bfseries 7.0 & 12.2 \\
 & 10 & 19.4 & 12.2 & \bfseries 7.0 & 15.2 \\
 & 20 & 15.8 & 12.4 & \bfseries 6.8 & 18.0 \\
\cline{1-6}
\multirow[c]{4}{*}{50} & 3 & 23.4 & 14.0 & \bfseries 8.6 & 16.0 \\
 & 5 & 28.8 & 14.6 & \bfseries 8.6 & 21.8 \\
 & 10 & 22.4 & 14.4 & \bfseries 7.0 & 21.0 \\
 & 20 & 15.8 & 13.8 & \bfseries 6.4 & 19.8 \\
\cline{1-6}
\bottomrule
\end{tabular}


==> tab/Median_n_steps_by_method.tex <==
\begin{tabular}{llrrrr}
\toprule
 &  & Picard & RGD & BWRAM & RCG \\
$d$ & $n_{\sigma}$ &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{3} & 3 & 27.0 & 30.3 & \bfseries 12.8 & 31.0 \\
 & 5 & 26.5 & 21.5 & \bfseries 13.8 & 24.5 \\
 & 10 & 23.3 & 15.8 & \bfseries 13.4 & 22.4 \\
 & 20 & 22.9 & 16.3 & \bfseries 13.3 & 26.1 \\
\cline{1-6}
\multirow[c]{4}{*}{5} & 3 & 72.1 & 33.3 & \bfseries 23.2 & 32.5 \\
 & 5 & 46.1 & 17.2 & \bfseries 13.5 & 24.5 \\
 & 10 & 41.8 & 16.6 & \bfseries 11.2 & 21.3 \\
 & 20 & 39.3 & 14.8 & \bfseries 10.0 & 22.1 \\
\cline{1-6}
\multirow[c]{4}{*}{10} & 3 & 120.9 & 25.2 & \bfseries 11.9 & 30.8 \\
 & 5 & 94.1 & 18.7 & \bfseries 10.3 & 26.7 \\
 & 10 & 89.7 & 15.6 & \bfseries 10.4 & 22.7 \\
 & 20 & 82.8 & 13.5 & \bfseries 9.8 & 16.5 \\
\cline{1-6}
\multirow[c]{4}{*}{20} & 3 & 245.7 & 23.9 & \bfseries 11.8 & 28.5 \\
 & 5 & 206.0 & 19.7 & \bfseries 11.3 & 30.5 \\
 & 10 & 192.8 & 18.5 & \bfseries 10.8 & 27.5 \\
 & 20 & 177.5 & 14.5 & \bfseries 10.6 & 14.8 \\
\cline{1-6}
\multirow[c]{4}{*}{50} & 3 & 707.5 & \bfseries 28.0 & 28.4 & 32.2 \\
 & 5 & 601.3 & \bfseries 22.8 & 26.5 & 35.1 \\
 & 10 & 506.9 & 25.8 & \bfseries 25.5 & 44.3 \\
 & 20 & 461.2 & 23.5 & \bfseries 20.5 & 40.5 \\
\cline{1-6}
\bottomrule
\end{tabular}


==> tab/OU_n_steps_by_method.tex <==
\begin{tabular}{llrr}
\toprule
 &  & Picard & BWRAM \\
$d$ & $\sigma_{max}$ &  &  \\
\midrule
\multirow[c]{4}{*}{2} & 1.0 & 15.0 & \bfseries 6.0 \\
 & 5.0 & 128.0 & \bfseries 11.0 \\
 & 10.0 & 250.0 & \bfseries 11.8 \\
 & 20.0 & 482.0 & \bfseries 15.0 \\
\cline{1-4}
\multirow[c]{4}{*}{4} & 1.0 & 20.0 & \bfseries 12.0 \\
 & 5.0 & 128.0 & \bfseries 22.0 \\
 & 10.0 & 250.0 & \bfseries 34.0 \\
 & 20.0 & 482.0 & \bfseries 69.5 \\
\cline{1-4}
\multirow[c]{4}{*}{8} & 1.0 & 21.0 & \bfseries 12.7 \\
 & 5.0 & 129.0 & \bfseries 37.8 \\
 & 10.0 & 251.0 & \bfseries 71.7 \\
 & 20.0 & 484.0 & \bfseries 106.0 \\
\cline{1-4}
\multirow[c]{4}{*}{16} & 1.0 & 22.0 & \bfseries 13.0 \\
 & 5.0 & 131.0 & \bfseries 33.3 \\
 & 10.0 & 255.0 & \bfseries 68.5 \\
 & 20.0 & 493.0 & \bfseries 115.7 \\
\cline{1-4}
\multirow[c]{4}{*}{32} & 1.0 & 23.0 & \bfseries 12.0 \\
 & 5.0 & 134.0 & \bfseries 38.2 \\
 & 10.0 & 262.0 & \bfseries 62.5 \\
 & 20.0 & 506.0 & \bfseries 113.3 \\
\cline{1-4}
\multirow[c]{4}{*}{64} & 1.0 & 24.0 & \bfseries 13.3 \\
 & 5.0 & 138.0 & \bfseries 37.0 \\
 & 10.0 & 270.0 & \bfseries 58.0 \\
 & 20.0 & 522.0 & \bfseries 106.8 \\
\cline{1-4}
\multirow[c]{4}{*}{128} & 1.0 & 25.0 & \bfseries 13.0 \\
 & 5.0 & 143.0 & \bfseries 33.7 \\
 & 10.0 & 278.3 & \bfseries 61.7 \\
 & 20.0 & 540.0 & \bfseries 103.3 \\
\cline{1-4}
\bottomrule
\end{tabular}

